Reachability via Compositionality in Petri nets

We introduce a novel technique for checking reachability in Petri nets that relies on a recently introduced compositional algebra of nets. We prove that the technique is correct, and discuss our implementation. We report promising experimental results on some well-known examples.

==> presround.tex <==
\begin{tabular}{| c || r | r | r | }
\hline
n  & time [s]\\ \hline
1 & 0.020 \\
2 & 0.300 \\
3 & 8.960 \\
4 & 105.930 \\
\hline
\end{tabular}

